PairUni: Pairwise Training for Unified Multimodal Language Models

Unified Vision-Language Models (UVLMs) perform both understanding and generation within a single architecture. Since these models rely on heterogeneous data and supervision, balancing both generation and understanding in reinforcement learning (RL) is challenging. To address this challenge, we propose PairUni, a unified framework that reorganizes data into understanding-generation (UG) pairs and aligns optimization accordingly. Specifically, we construct a unified paired dataset by synthesizing aligned instances via cross-modal semantic completion and retrieving semantically related samples. These paired structures expose cross-task semantic correspondences and support consistent policy learning. To leverage this structure, we present PairGRPO, a pair-aware variant based on Group Relative Policy Optimization. It assigns a similarity score to each pair to modulate the advantage, strengthening learning from well-aligned examples and reducing task interference. Extensive experiments across diverse UVLM architectures (Autoregressive and Discrete Diffusion) and scales (1B to 14B) demonstrate that PairUni yields consistent improvements over strong baselines. Notably, our method also demonstrates strong generalization by improving performance on image editing tasks without using any editing-specific data. Codes are available at https://github.com/Haochen-Wang409/PairUni.

==> sections/2-relatedwork.tex <==
\section{Related Work}
\label{app:related_work}


\noindent 
\textbf{Unified Vision-Language Model.}
The pursuit of unified multimodal frameworks has led to significant innovations in both architecture design and training paradigms. 
Early approaches~\cite{xie2024showo,team2024chameleon} like Show-o series~\cite{xie2024showo,xie2025showo2} establish the autoregressive foundations for joint vision-language processing.
Meanwhile, Transfusion~\cite{zhou2025transfusion} introduces diffusion-based methodologies to enhance generation quality. 
These foundational works, as systematically analyzed in~\cite{zhang2025unifiedmultimodalunderstandinggeneration}, demonstrate the potential of unifying modalities through shared representation learning.
Recent advances have pushed the boundaries of unified modeling~\cite{deng2025bagel,chen2025janusprounifiedmultimodalunderstanding}. 
For example, Janus-Pro~\cite{chen2025janusprounifiedmultimodalunderstanding} innovatively uses bidirectional encoder-decoder structures for understanding and generation, achieving stronger performance on both sides.
Bagel~\cite{deng2025bagel} adopts transformer experts and is trained with massive image generation and understanding data, leading to the state-of-the-art performance.
This architectural evolution aligns with the broader trend of developing modular yet integrated systems that can dynamically adapt to different modalities.
In this context, our work enhances UVLMs post-training, in particular, during the reinforcement learning phase. 
We present a novel view of pair data generation and utilization of such pair data with proposed Pair-GRPO.


\noindent
\textbf{Reinforcement Learning in UVLMs.} The integration of reinforcement learning (RL) has emerged as a critical component for advancing unified MLLMs during the post-training. 
Early RL applications focused on modality-specific enhancements: step-by-step rule-based rewards for mathematical reasoning~\cite{shao2024deepseekmathpushinglimitsmathematical}, and bbox IoU rewards for visual grounding~\cite{jiang2025t2i}. 
For text-to-image generation, CLIP-based rewards~\cite{radford2021learning} became standard for aligning visual outputs with textual descriptions. 
The paradigm shifted with unified RL approaches that exploit cross-modal synergies. 
T2I-R1~\cite{jiang2025t2i} pioneered iterative refinement through GRPO~\cite{shao2024deepseekmathpushinglimitsmathematical}, using detailed descriptions as intermediate rewards. 
Recently, several works also explore the RL-based post-training for UVLMs.
In particular, UniRL~\cite{mao2025unirlselfimprovingunifiedmultimodal} proposed a self-improving pipeline where generated QA pairs simultaneously serve as training data and reward signals, though this approach showed performance degradation in understanding benchmarks. 
More sophisticated reward mechanisms have since been developed. DSR~\cite{hong2025reinforcing} introduced dual-source rewards combining original image-caption pairs with generated content, while HermesFlow~\cite{yang2025hermesflowseamlesslyclosinggap} implemented Pair DPO~\cite{rafailov2024directpreferenceoptimizationlanguage} to enforce consistency between modalities. 
Notably, CoRL~\cite{jiang2025coreinforcementlearningunifiedmultimodal} adopts a two-stage approach, first training unified RL on shared data before specializing in understanding/generation phases, demonstrating improved performance across multiple benchmarks.
Different from these methods, which all focus on unified RL method design, our work provides a new view on understanding data and generation data.
We propose to build the UG pairs to benefit both tasks.
With proposed Pair-GRPO along with UG pairs, our work improves various UVLMs.

==> sections/statement.tex <==
\label{app:statement}

\section*{The Use of Large Language Models}
We used a Large Language Model (LLM) only as a writing assistant to polish the language of the manuscript (e.g., grammar refinement, style adjustment, and clarity improvement). The research ideas, methodology design, experiments, and analysis were entirely conceived, implemented, and validated by the authors without reliance on the LLM. The LLM did not contribute to research ideation, experimental design, or result interpretation.

==> tables/ablation_sim.tex <==
\begin{table}[t]
    \vspace{-1em}
\centering
\caption{\textbf{Ablation study on Trajectory-level credit assignment.}}
\label{tab:sim}
\scalebox{0.7}{
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Model} & \textbf{MME(P)} & \textbf{MMMU} & \textbf{MMStar} & \textbf{GenEval} \\
        \midrule
        PairUni-1B w/o sim & 1469.87 & 40.0 & 45.1 & 0.79 \\
        \rowcolor{cyan!5}
        PairUni-1B & \textbf{1483.18} & \textbf{40.4} & \textbf{46.1} & 0.79 \\
        \hdashline
        PairUni-7B w/o sim & 1554.91 & 47.0 & 47.7 & 0.85 \\
        \rowcolor{cyan!5}
        PairUni-7B & \textbf{1597.71} & 47.0 & \textbf{49.5} & 0.85 \\
        \bottomrule
    \end{tabular}
}
\vspace{-1em}
\end{table}

==> tables/more_results_del.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Additional Model Validations.} Results of SFT experiments on BAGEL and the application of the PairUni method on Lumina-DiMOO using PairUG-16k data. The table confirms the generalizability of the proposed approach across different model architectures.}
\scalebox{0.80}{
\begin{tabular}{lcccc|c}
\toprule
\textbf{Model} & \textbf{MME(P)} & \textbf{MMMU} & \textbf{MMStar} & \textbf{POPE} & \textbf{GenEval}\\
\midrule
Lumina-DiMOO & 1534.2 & 58.6 & 52.4 & 87.4 & 0.88 \\
\rowcolor{cyan!5}
\textbf{Lumina-DiMOO~\cite{lumina-dimoo} w PairUni} & \textbf{1551.8} & \textbf{61.3} & \textbf{52.6} & \textbf{87.5} & \textbf{0.89} \\
\hdashline
BAGEL & 1687.0 & 55.3/52.8$^{*}$ & - & 87.4$^{*}$ & 0.82/0.78$^{*}$ \\
\rowcolor{cyan!5}
\textbf{BAGEL~\cite{deng2025bagel} + SFT} & 1642.0 & \textbf{53.7} & - & \textbf{87.7} & \textbf{0.79} \\
\bottomrule
\end{tabular}}
\label{tab:more_model}
\\[2pt]
\footnotesize{$^{*}$ Results obtained from the publicly released checkpoint rather than the original reported numbers.}
\vspace{-1em}
\end{table*}


